A Variability Fault Localization Approach for Software Product Lines

Software fault localization is one of the most expensive, tedious, and time-consuming activities in program debugging. This activity becomes even much more challenging in Software Product Line (SPL) systems due to variability of failures. These unexpected behaviors are induced by variability faults which can only be exposed under some combinations of system features. The interaction among these features causes the failures of the system. Although localizing bugs in single-system engineering has been studied in-depth, variability fault localization in SPL systems still remains mostly unexplored. In this article, we present VarCop, a novel and effective variability fault localization approach. For an SPL system failed by variability bugs, VarCop isolates suspicious code statements by analyzing the overall test results of the sampled products and their source code. The isolated suspicious statements are the statements related to the interaction among the features which are necessary for the visibility of the bugs in the system. The suspiciousness of each isolated statement is assessed based on both the overall test results of the products containing the statement as well as the detailed results of the test cases executed by the statement in these products. On a large dataset of buggy SPL systems, empirical evaluation shows that VarCop significantly improves two state-of-the-art fault localization techniques by 33% and 50% in ranking the incorrect statements in the systems containing a single bug each. In about two-thirds of the cases, VarCop ranks the buggy statements at the top-3 positions in the resulting lists. For multiple-bug cases, VarCop outperforms the state-of-the-art approaches 2 times and 10 times in the proportion of bugs localized at the top-1 positions. In 22% and 65% of the buggy versions, VarCop correctly ranks at least one bug in a system at the top-1 and top-5 positions.

==> 5.feature_interaction/5.2.root_cause_old.tex <==



\subsection{The Root Cause of Variability Failures}
\label{sec:root_cause}
The variability bugs in an SPL system can be revealed by multiple sets of the features which must be enabled and disabled \textbf{together} to make the bugs visible in the system. 
For each of these set of the relevant features, their selection might affect the visibility of the bugs in the system. 
%
% Thus, in this paper, we consider that each such set of features as a root cause of the failures in the system.
%

Let first consider the cases where the failures of a system is revealed by a single set of the relevant features, $F_r = F_E \cup F_D$, where the features in $F_E$ and $F_D$ must be respectively enabled and disabled \textbf{together} to make the bugs visible.
%
Specially, the features in $F_E$ and $F_D$ must be respectively on and off in all failing products.
%
From a failing product $p \in P_F$, when switching the current selection of any switchable features in $F_r$, the resulting product $p'$ will pass all its tests, $p' \in P_P$. The relation between the variability bugs and the interaction between the features in $F_r$ will be theoretically discussed as following.

Let $\mathcal{S}$ be the set of buggy statements which cause the failures in product $p \in P_F$.
%
From the current configuration of $p$, disabling any feature $f_e \in F_E$ makes the resulting product, $p'$, passes all its tests. We have two following cases.
%
First, the buggy statements are \textit{not present} in $p'$, $\mathcal{S} \subseteq \varphi(f_e)$. Since, $\varphi(f_e) \subseteq \alpha(f_e, p)$, thus, $\mathcal{S} \subseteq \alpha(f_e, p)$.
%
The second case is that the statements in $\mathcal{S}$ are present in $p'$, yet \textit{behave differently} from the way they do incorrectly in $p$ because of the absence of the impact of feature $f_e$ on $\mathcal{S}$. It means, $\mathcal{S} \subseteq \alpha(f_e, p)$. This causes the unexpected behaviors of the incorrect statements do not expose in $p'$.
%
These cases demonstrate, $\forall f_e \in F_E, \mathcal{S} \subseteq \alpha(f_e, p)$. Therefore, $\mathcal{S} \subseteq \beta(F_E, p) = \bigcap_{f_e\in F_E} \alpha(f_e, p)$. 
%
In other words, \textit{the set of the incorrect statements $\mathcal{S}$ is a part of the implementation of the interaction among the features in $F_{E}$} (Mentioned in \textbf{O1}).


%They can question about this about feature model. Let them ask!!!
In addition, from $p$, turning on any disabled feature $f_d \in F_D$, the resulting product $p''$ also passes all its tests. The reason is, the presence of $f_d$ makes the buggy statements behave differently in $p''$. In other words, the statements in $\mathcal{S}$ are impacted by $f_d$ in $p''$, $\mathcal{S} \subseteq \alpha(f_d, p'')$. Intuitively, the presence of $f_d$ has an impact on the way features $F_E$ interact with each other. Therefore, the buggy statements in $\mathcal{S}$ cannot behave incorrectly as when they do in $p$ because of the presence of the impact of $f_d$ in $p''$.
Hence, \textit{there is an interaction among the features in $F_E \cup \{f_d\}$ in $p''$, and the set of the incorrect statements $\mathcal{S}$ is a part of this interaction, $\mathcal{S} \subseteq \beta(F_E \cup \{f_d\}, p'')$} (Mentioned in \textbf{O2}).

Overall, the interaction among the features in $F_{E}$ and $F_{D}$ is the root cause of the failures caused by variability bugs. Thus, identifying the sets of the features such that the presence/absence of their interactions makes the bugs visible/invisible and the implementation of these interactions is necessary to localize variability bugs in SPL systems. 

% Note that, without loss of generality, a feature can interact with itself and the base code (i.e. features which are compulsorily enabled) is considered as a feature of the system.

In general, variability bugs in a system can be revealed by multiple root causes. In these cases, the visibility of the bugs might not be clearly observed by switching the selections of features in one set of relevant features. For instance, $F_r$ and $F_r'$ are two sets of relevant features whose interaction causes the failures in the system. Once switching the selection of any feature in $F_r$, the implementation of the interaction among the features in $F_r$ is not in the resulting product $p'$. Meanwhile, $p'$ can still contain the interaction among the features in $F_r'$. Thus, $p'$ can still fail some tests. 
However, if we can identify $F_r$ and/or $F_r'$ or even their subsets, by examining the interaction among the identified set(s) of features, the bugs are still be isolated. More details will be described and proved in the next Section.


==> 9.eval/9.1.bug_generation.tex <==
\subsubsection{Variability Bug Generation}
\label{sec:single_bug_generation}
Since constructing a dataset of the real variability bugs with the corresponding tests is a considerable task, until now there is no such public dataset.
% for variability bugs with the corresponding tests. 
Additionally, the existing work~\cite{just2014mutants} has shown that the performance of FL techniques on real bugs can be estimated based on their performance on artificial bugs. Thus, we evaluate {\tool} on a dataset of artificial variability bugs which are systematically generated in three main steps: \textit{Product Sampling and Test Generating}, \textit{Bug Seeding}, and \textit{Variability Bug Verifying}.
%
% \begin{figure}
%     % \centering
%       \includegraphics[width=1.00\linewidth]{Image/bug_generation.png}
%     \caption{Variability bug generation procedure }
%     \label{fig:bug_generation}
% \end{figure}

\textbf{\textit{Step 1} - Product Sampling and Test Generating.}
%Sampling
Firstly, for an SPL system, a set of the products of the system is systematically sampled by the existing techniques~\cite{sampling_comparision, kwise2012}. Particularly, we sample a set of the valid configurations with the $k$-wise coverage by \textit{SPLCA tool}~\cite{kwise2012}. 
%
For each configuration, the corresponding product is composed. 
%Test generation
For each product $p$, a test suite is generated using existing test generation techniques to capture the original behaviors of $p$. 
%
In this work, we use \textit{Evosuite}~\cite{fraser2011evosuite} to generate tests.
% which is a popular search-based method and widely used to automatically generate tests. 
% Additionally, \textit{Evosuite} can generate and optimize the whole test suites towards satisfying a coverage criterion.
%
% \textit{Evosuite} is run over each sampled product to capture the original behaviors of the product. 
% Also, these behaviors are test oracle, because the original system is considered as bug-free.
For each test of $p$, the output will be recorded and used as the test oracle of the corresponding test in the product having the same configuration as $p$ in the mutated system in \textit{Step 2}.


\textbf{\textit{Step 2} - Bug Seeding.} A modification is \textit{randomly} seeded into a system by using a mutation operator. 
We use $\mu$\textit{Java}~\cite{ma2006mujava}. 
% $\mu$\textit{Java} seeds faults by using mutation operators
% such as \textit{arithmetic operator replacement} or \textit{conditional operator insertion} 
% to modify the source code of the system. 
%
These mutations change the original behaviors of the several products which are expected to be captured by the tests and make their current outputs different from the outputs recorded in \textit{Step 1} (i.e., failing tests). 

\textbf{\textit{Step 3} - Variability Bug Verifying.} Finally, to ensure that the seeded bugs are variability bugs that can be caught by the tests, the collection of products of the mutated system, which are corresponding to the same configurations selected in \textit{Step 1}, are re-selected. 
% This means that each seeded bug of the system is settled in the corresponding products. 
After that, we run each product against its test suite. 
% The product is a failing product if at least one of its tests fails, otherwise, it is a passing product. 
\textit{A bug is considered as a variability bug if it causes the failures in certain sampled products}. In other words, after testing the mutated system, the sampled set of products contains both the passing and failing products.
%
% Additionally, the test information is required for fault localization process, and, they are recorded by \textit{OpenClover} \cite{?} during tests run.

\subsubsection{Multiple Variability Bugs Generation}


We also systematically create a dataset containing the versions of the subject systems such that each version consists of multiple variability bugs. To do that, we extend \textit{Step 2} and \textit{Step 3} in Sec.~\ref{sec:single_bug_generation} to generate such dataset as follows: 

\textbf{Multiple Bugs Seeding}. In \textit{Step 2}, instead of applying a single modification as in the cases of a single bug, a random number, $n > 1$, of mutation operators are continuously used to mutate the source code of the system.

\textbf{Variability Bugs Verifying}. In \textit{Step 3}, all the bugs need to be verified to ensure that they are all variability bugs. Particularly, \textit{when one or more bugs are fixed, the remaining bugs still cause the failures in certain products}. In other words, unless all the bugs are fixed, there still exists both the passing and failing products. We aim to simulate the bug-fixing process by developers in practice. That is, for each case, we gradually fix each bug by reverting the modification to the original state and do regression testing. 
%
The case would be accepted if there still exists both the passing and failing products until
all the bugs are fixed.
%


%We might miss the case where variability bugs and normal bugs are mixed. But, it's ok. Let's see how people think, then we will add that part if requested.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

